Envisioning New Futures of Positive Social Technology: Beyond Paradigms of Fixing, Protecting, and Preventing

Social technology research today largely focuses on mitigating the negative impacts of technology and, therefore, often misses the potential of technology to enhance human connections and well-being. However, we see a potential to shift towards a holistic view of social technology's impact on human flourishing. We introduce Positive Social Technology (Positech), a framework that shifts emphasis toward leveraging social technologies to support and augment human flourishing. This workshop is organized around three themes relevant to Positech: 1) "Exploring Relevant and Adjacent Research" to define and widen the Positech scope with insights from related fields, 2) "Projecting the Landscape of Positech" for participants to outline the domain's key aspects and 3) "Envisioning the Future of Positech," anchored around strategic planning towards a sustainable research community. Ultimately, this workshop will serve as a platform to shift the narrative of social technology research towards a more positive, human-centric approach. It will foster research that goes beyond fixing technologies to protect humans from harm, to also pursue enriching human experiences and connections through technology.

==> inputs.tex <==
\begin{figure}[t]
    \centering
    \thispagestyle{empty}
    \includegraphics[width=0.8\linewidth]{venn_diagram.jpg}
    \caption{Venn Diagram of Positech and Related Concepts}
    \Description {The image depicts a Venn diagram with three overlapping circles within a larger rectangular frame titled ``Positech.'' Each circle represents a different field: ``Positive Technology,'' ``Positive Computing,'' and ``Asset-based Approach.'' The overlapping sections of the circles are labeled with letters (A), (B), (C), (D), and (E) to indicate areas of intersection between these fields. Area (A) is the portion of the ``Positive Technology'' circle that does not overlap with the other fields. Area (B) is the portion of the ``Positive Computing'' circle that does not overlap with the other fields. Area (C) is the portion of the ``Asset-based Approach'' circle that does not overlap with the other fields and is outside of the ``Positech'' rectangle. Area (D) is the portion within Positech that is outside the all other circles, indicating the unique portion of the ``Positech'' rectangle. Area (E) is the central overlapping area where all three circles intersect, indicating a shared space between ``Positive Technology,'' ``Positive Computing,'' and ``Asset-based Approach.''}
    \label{fig:venn_diagram}
\end{figure}

